SAT-Based Extraction of Behavioural Models for Java Libraries with Collections

Behavioural models are a valuable tool for software verification, testing, monitoring, publishing etc. However, they are rarely provided by the software developers and have to be extracted either from the source or from the compiled code. In the context of Java programs, a number of approaches exist for building behavioural models. Most of these approaches rely on the analysis of the compiled bytecode. Instead, we are looking to extract behavioural models in the form of Finite State Machines (FSMs) from the Java source code to ensure that the obtained FSMs can be easily understood by the software developers and, if necessary, updated or integrated into the original source code, e.g. in the form of annotations. Modern software systems are huge, rely on external libraries and interact with their environment. Hence, extracting useful behavioural models requires abstraction. In this paper, we present an initial approach to this problem by focusing on the extraction of FSMs modelling library APIs. We focus on the analysis of Java code involving the use of collections. To this end, we encode the operational semantics of collection operations using patterns of Boolean predicates. These patterns are instantiated based on the analysis of the source code of API implementation methods to form an encoding of the possible FSM transitions. A SAT solver is then used to determine the enabledness conditions (guards) of these transitions.

==> src/collections.tex <==
\subsection{General purpose implementations}
We based our tool on Java Collection Framework of the last version at the moment (JDK 17)~\cite{javacollections} and we were interested in its General Purpose Implementations (GPI) presented in the table below. 

\begin{table}[!ht]
\tiny
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 Implementation Style / Interface & Set & List & Queue, Deque & Map \\ 
 \hline
 HashTable & HashSet & & & HashMap \\
 ResizableArray & & ArrayList & ArrayDeque &  \\
 BalancedTree & TreeSet & & & TreeMap \\
 LinkedList & & LinkedList & LinkedList & \\
 HashTable + LinkedList & LinkedHahSet & & & LinkedHashMap \\
\hline
\end{tabular}
\end{table}

For all GPI, we  divided their methods to the ones changing the state (add, remove, etc.) and the ones retrieving information (size, empty, etc). We need the first to generate predicates capturing changes of the collection state, and the second to analyze the state of collection and involved variables, e.g in conditional expressions.

We studied each GPI to capture its behaviour to define its operational semantics taking into account differences in the implementation of methods for various interfaces.

\subsubsection{Set}
Except from the main property of (1) having no duplicates, other properties we are taking into account are (2) if the collection is ordered (no/yes  with natural order or by comparator / yes with insertion order), and (3) if it permits null values. 
From the point of view of predicate abstraction, we could neglect the collection's initial capacity and load factor (as the operation of
enlarging the collection happens implicitly), and the insertion order (since retrieving elements is not based on their position in the collection). These assumptions allow us to treat the HashSet and the LinkedHashSet equally. For the TreeSet we have extra rules for adding and removing null elements and for constructors capturing the behaviour lacking in the HashSet and the LinkedHashSet collections.

\subsubsection{List}
List is an ordered collection, allowing duplicates and null values. List implemetations varies depending on its possibility to be sychronised (Vector
and Stack contra ArrayList and LinkedList) which is a negligibale distinction for our purposes.

\subsubsection{Queue, Deque}
The only general purpose implementation is ArrayDeque. It is resizeable with not capacity restrictions, not thread-safe,
with null elements being prohibited. From the point of view of methods, ArrayDeque is similiar to the LinkedList, but it
does not support operations based on the index (e.g add(e,e), set(i,e), remove(i,e)). Adding operations here are divided
into those adding to the front or the end of the queue. Removing operations can remove an object placed anywhere, but
also divided into two groups depending if they throw NoSuchElementExceptionn on the empty collection or not.

\subsubsection{Map}
Map is a special type of collections not inhereted from Collection interface

\subsection{Operational semantics}



==> src/future.tex <==
In this section we present the current challenges for the tool and our thought on resolving them.

\subsubsection{Combining models}

\subsubsection{Dealing with language challenges}
The nature of the code poses several challenges for the tool: not all functions can be evaluated (e.g due to infinite behaviour), lambda functions,  functions with random behaviour, static fields and reflection, etc. \todo{super! so what do we do?}

There are at least several cases, where receiving extra information from use can enhance the model. E.g if the tool can't infer the type hierarchy for exceptions and therefore can't build CFG fully reflecting it, we can solve the problem by annotating the code with the missing information:
\begin{lstlisting}
void foo() throws OneException /* extends OtherException */
\end{lstlisting}
Another solution could be inquiring missing information from user after detecting the problem and rebuild the model.

\subsubsection{Automata optimization}
automata minimization + automata bisimilation

\subsubsection{Step to distribution}
combining and coordination of extracted models

runtime monitoring based on extracted models

JavaBIP + verification of extraction models
need annotations for program proof 
 

%Example: For the code below we will have CFG1 if we know that SomeException extends OtherException or CFG2 if we don't.
%\begin{lstlisting}
%public void do() throws SomeException { 
%    status = DONE;
% } 
%
%public void test() {
%    status = NEW;
%    try {
%        do();
%    } catch (OtherException e) {
%        status = RECOVERY;
%    }
%    finally {
%        status = FINAL;
%    }
%}
%\end{lstlisting}

==> src/introduction.tex <==
\textbf{TODO: HERE WE ADVOCATE THAT BEHAVIORAL MODELS ARE COOL}


Source code behavioral models are beneficial for the program verification and testing \cite{10.1145/332740.332741}, coordination and monitoring \cite{} and for many other applications, which makes extracting a behavioral model desirable but not a trivial goal.

Behavioral models

Usage: 
1)breaking changes
2) static aalysis monitoring coordination


Reusing components, such as libraries and API helps to reduce the cost of software systems development and to increase their quality~\cite{Espinha2015WebAG, brito17, brito18}. However, external libraries and API being a black box are representing error-prone dependencies and making such systems prone to breaking changes that have to be addressed in the client code. A new version of an external interface evolving independently could break backward compatibility and may cause the runtime failure of a client system. 

The problem of introducing breaking changes is well-studied in literature~\cite{RAEMAEKERS2017140, dietrich14, dig06} which shows it could be represented in the significant amount of all new releases (70\% according to Raemaekers et al, 75\% according to Dietrich et al, and 80\% according to Dig et al). To detect the problem, two releases are being compared for having binary or source compatibility. For example, in~\cite{RAEMAEKERS2017140} Raemaekers et al have studied the history of more than 22000 libraries in the Maven Central repository from the point of view of their binary compatibility. And in~\cite{dig06} Dig et al has introduced the algorithm and the tool for studied source incompatibility introduced by refactoring in Java code (renaming, moving, and changing signature). This tool combines syntactic and semantic code analysis comparing the body of methods and call graphs in the source with the target, identifying the same methods and methods being deleted or introduced, changed or moved, etc.

Our approach in supporting the process of identifying breaking changes lies in generating behavioural models based on the API source code. 

In this paper we present our approach to semi-automatic extraction of behavioural models in the form of Finite State Machines, made for Java source code. The paper is structured as follows. In~\autoref{chap:example} we present a running example based on the Java Remote Method Invocation framework and explain our approach in \autoref{chap:tool}. \autoref{chap:others} covers the related works, \autoref{chap:future} explores future research directions and \autoref{chap:final} draws conclusions.  
% There exist several models allowing graphical representation of the code (AST, CFG, FCG others, describe them)
% Especially if the code is concurrent (links)
% There exist many formal models for concurrent code (choreographies and stuff)
%\subsection{Model applications}
%java bip spec generation, models for existing api (changes etc) how to use them? if they represent what you want? documenting code, conformance to requierements
%why:using model in different contexts ,use model (e.g java-bip, other applications)

==> src/relatedWork.tex <==
\subsection{Behavioral models}
In~\cite{lorenzoli18} authors use the similiar approach of building the model both on the data constraits and iteraction between components. They have presented the technique called GK-tail to generate automatically extended FSM from program's interaction traces taking into account constraints on data values. 


\subsection{CFG}
Although some tools for building CFGs of Java programs do exist \cite{ Amighi2012,DJN14,progex,dragon05,liva2017pcfg,codehawk20}, %
most operate on Java bytecode.  Instead, we do so directly
at the Abstract Syntax Tree (AST) level to avoid the high-level
abstractions being compiled away during the translation to
intermediate code \cite{Soderberg13}. Indeed, while most tools build
CFG for analysis purposes, e.g formal verification, we aim at
establishing a connection between the extracted model and the source
code.

Mungo, uml, famelis
automatic and semi-automatic models

manual models

michalis famelis "api and automata" formalise 2021


bytecode analysis

static analysis

formal models (chor extraction?)



==> src/tool.tex <==
\subsection{Architecture}
The proposed tool should be able to build a model for both basic types (numerical types like integers and floats of both primitive and of Object types, booleans, strings and enumerations) and collections. 
In general, the algorithm follows these steps: (1) collecting the information on sources under analysis and the property which state changes we explore, (2) computing auxiliary data structures, and collecting all easily evaluating values of states, (3) using different techniques of static and runtime code analysis to generate FSM. The last step differs for the basic types and collections, and as our main goal is to deal on the latest, we will focus on our approach of using the SAT-based analysis.

\begin{figure}[h]
 \caption{Main phases: (1) collecting sources and extraction information, (2) creating auxiliary structures, (3) using SAT-based analysis to produce FSM}
 \centering
 \includegraphics[width=0.45\textwidth]{src/context.png}
\end{figure}


\subsection{SAT-based Analysis for Collections}
To manipulate with the collection we define a context and a pattern. The context contains a fixed variable v and variables passed as signature parameters which were involved in manipulations with the collection. The pattern consists of predicates capturing the lifecycle of the context variables. The predicates could be:
\begin{enumerate}
    \item Class scope: 
    \begin{itemize}
        \item The default predicate for the fixed value: b0 = c.contains(v)
        \item Predicates for all values that can be evaluated statically:  b1 = v == “hello world!”
        \item Predicate for expressing exceptional behavioural: exc
    \end{itemize}
    \item Function scope predicates for local variables and signature parameters involved in actions with the collection capturing: 
    \begin{itemize}
        \item the state required for the rules of operational semantics for the selected collection: c1 = c.contains(n1) (for all sets), c2 = v == null (for TreeSet)
        \item presence in the collection: c1 = c.contains(n1)
        \item equational relation between two variables: p1 = n1 == value, p2 = n1 == n2
        \item condition behaviour: c1 = n1 != null
    \end{itemize}
    \item More complicated predicates for the actions on the collection defined by the operational semantics

\end{enumerate}




Class-scope predicates can be calculated statically and they form the states of the future FSM. Function-scope predicates can be calculated only dynamically and they define the guards of the FSM’s transitions.

\subsection{Java collections}
\label{chap:collections}
\input{src/collections}

